Latent Unexpected and Useful Recommendation

Providing unexpected recommendations is an important task for recommender systems. To do this, we need to start from the expectations of users and deviate from these expectations when recommending items. Previously proposed approaches model user expectations in the feature space, making them limited to the items that the user has visited or expected by the deduction of associated rules, without including the items that the user could also expect from the latent, complex and heterogeneous interactions between users, items and entities. In this paper, we define unexpectedness in the latent space rather than in the feature space and develop a novel Latent Convex Hull (LCH) method to provide unexpected recommendations. Extensive experiments on two real-world datasets demonstrate the effectiveness of the proposed model that significantly outperforms alternative state-of-the-art unexpected recommendation methods in terms of unexpectedness measures while achieving the same level of accuracy.

==> Reproducible.tex <==
\section{Pseudo Code for Unexpected Recommendation}

\begin{algorithm}
\SetAlgoLined
\KwData{Heterogeneous Information Network (HIN)}
\KwResult{Lists of Recommended Items}
\For{each node $e$ in HIN}{HeterogeneousRandomWalk(e)}
Heterogeneous-Node2Vec(HIN)\;
\For{each user $u$ in HIN}{
\For{each item $i$ in HIN}{
Unexpectedness($u$, $i$) = Distance(Convex-Hull($u$), $i$)\;
Utility($u$, $i$) = $\alpha$*Unexpectedness($u$, $i$) + (1-$\alpha$)*Rating($u$, $i$)}
Recommend TopN(Utility)\;}
 \caption{Latent Unexpected Recommendation}
\end{algorithm}

\section{Hyperparameter Settings}
We perform the optimization method to select the best hyperparameters for our proposed model. The hyperparameters for the heterogeneous random walk are selected as follows:
\begin{itemize}
\item Numbers of walks per node: 10
\item Walk length: 100
\end{itemize}

The hyperparameters for the skip-gram mechanism are selected as follows:
\begin{itemize}
\item Embedding dimension: 128
\item Window size: 2
\item Minimal term count: 1
\item Iterations: 100
\item Workers: 1
\end{itemize}

For the unexpected recommendations, we perform 5-fold cross-validation evaluation and average the performance values.

\section{Dataset and Implementation}
We use two publicly-available datasets for the experiment, the Yelp Challenge Dataset Round 12 (https://www.yelp.com/dataset/challenge) and the TripAdvisor Dataset (http://www.cs.cmu.edu/~jiweil/html/hotel-review.html). The recommendation model is implemented in the Python environment using the ''Surprise'' package. The convex hull is computed using the ''SciPy'' package. The skip-gram mechanism is implemented using the ''Gensim'' package. The codes will be available upon acceptance of this paper, for we can not share them here due to anonymity.

